LLMCad: Fast and Scalable On-device Large Language Model Inference

Generative tasks, such as text generation and question answering, hold a crucial position in the realm of mobile applications. Due to their sensitivity to privacy concerns, there is a growing demand for their execution directly on mobile devices. Currently, the execution of these generative tasks heavily depends on Large Language Models (LLMs). Nevertheless, the limited memory capacity of these devices presents a formidable challenge to the scalability of such models. In our research, we introduce LLMCad, an innovative on-device inference engine specifically designed for efficient generative Natural Language Processing (NLP) tasks. The core idea behind LLMCad revolves around model collaboration: a compact LLM, residing in memory, takes charge of generating the most straightforward tokens, while a high-precision LLM steps in to validate these tokens and rectify any identified errors. LLMCad incorporates three novel techniques: (1) Instead of generating candidate tokens in a sequential manner, LLMCad employs the smaller LLM to construct a token tree, encompassing a wider range of plausible token pathways. Subsequently, the larger LLM can efficiently validate all of these pathways simultaneously. (2) It employs a self-adjusting fallback strategy, swiftly initiating the verification process whenever the smaller LLM generates an erroneous token. (3) To ensure a continuous flow of token generation, LLMCad speculatively generates tokens during the verification process by implementing a compute-IO pipeline. Through an extensive series of experiments, LLMCad showcases an impressive token generation speed, achieving rates up to 9.3x faster than existing inference engines.

==> fig-auto-regressive.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/auto-regressive.pdf}
	\caption{The overview of LLM inference pattern: auto-regressive.\xdl{merge Figure 1 and 2 later.}}
	\label{fig-auto-regressive}
\end{figure}

==> fig-inferece-model-energy.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/figure-model-inference-orin-energy.pdf}
        \caption{Jetson Orin}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/figure-model-inference-tx2-energy.pdf}
        \caption{Jetson TX2}
    \end{subfigure}
    
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/figure-model-inference-xiaomi11-energy.pdf}
        \caption{Xiaomi 11}
    \end{subfigure}
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figs/figure-model-inference-xiaomi10-energy.pdf}
        \caption{Xiaomi 10}
    \end{subfigure}

    \caption{The energy consumption of different models across different devices.}
    \label{figure-inference-model-energy}
\end{figure}

==> fig-inference-large-utilization.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figs/figure-large-inference-utilzation.pdf}
    \caption{The GPU utilization on TX2 when inferring the \largemodel model using PyTorch.}
    \label{fig-large-inference-utilization}
\end{figure}

==> fig-masking.tex <==
\begin{figure}
    \centering
    \subfigure[Masking table]{\includegraphics[width=0.2\textwidth]{figs/masking.pdf}}
    \subfigure[Tree masking table]{\includegraphics[width=0.25\textwidth]{figs/tree-masking.pdf}}
    \caption{(a) Masking table in state-of-the-art DL engines and its effects. (b) The tree masking table of the example token tree in Figure~\ref{fig-kv-cache-default} used in \sys. }
    \label{fig-masking}
\end{figure}

==> fig-model-size-accu-latency.tex <==
\begin{figure}
    \centering
    \subfigure[SQuAD on TX2 (1GB budget)]{\includegraphics[width=0.23\textwidth]{figs/figure-model-size-accu-latency.pdf}}
    \subfigure[TriviaQA on Xiaomi10 (6GB budget)]{\includegraphics[width=0.23\textwidth]{figs/figure-model-size-accu-latency-phone.pdf}}
    \caption{The accuracy on the question answering datasets and inference latency of LLM models with model size increasing. Solid line: accuracy. Dash line: inference latency. \xdl{add other LLMs on the phone later}}
    \label{fig-model-size}
\end{figure}

==> table-accuracy-task-smartphone.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \resizebox{0.96\textwidth}{!}{%
% \begin{tabular}{@{}lrr|r|rrr@{}}
% \toprule
% \textbf{}                          & \multicolumn{2}{c|}{\textbf{Vicuna-13B-INT4}}   & \multicolumn{1}{c|}{\textbf{Vicuna-33B-INT4}} & \multicolumn{3}{c}{\textbf{LLaMa2-Chat-INT4}}                                         \\ \midrule
% \textbf{}                          & \multicolumn{1}{r|}{T: Parrot} & T: WMT22-de-en & T: WMT22-zh-en                                & \multicolumn{1}{r|}{S: CNN/Daily} & \multicolumn{1}{r|}{QA: SQuAD} & QA: Truthful\_QA \\ \midrule
% \multicolumn{1}{l|}{\textbf{STI}}  & \multicolumn{1}{r|}{100}       & 100            & 100                                           & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{100}       & 100              \\
% \multicolumn{1}{l|}{\textbf{BLD}}  & \multicolumn{1}{r|}{89.7}      &        90.2      &                     88.4                       & \multicolumn{1}{r|}{60.4}             & \multicolumn{1}{r|}{3.4}        &          4.7     \\
% \multicolumn{1}{l|}{\textbf{Ours}} & \multicolumn{1}{r|}{100}       & 100            & 100                                           & \multicolumn{1}{r|}{100}          & \multicolumn{1}{r|}{100}       & 100              \\ \bottomrule
% \end{tabular}%
% }
% \caption{The summary of the relative similarity to the \largemodel LLM of \sys and the baseline on smartphones. T:*, S:*, and QA:* represent the generative tasks of translation, summary and question-answering.}
% \label{table-accuracy-tasks-smartphones}
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llrrr}
% \hline
% \textbf{Model}                             & \textbf{Dataset} & \textbf{STI} & \textbf{BLD} & \textbf{Ours} \\ \hline
% \multirow{3}{*}{\textbf{Vicuna-13B-INT4}}  & T: Parrot        & 100          & 89.7         & 100           \\
%                                            & T: WMT22-de-en   & 100          & 90.2         & 100           \\
%                                            & T: WMT22-zh-en   & 100          & 80.4         & 100           \\ \hline
% \multirow{3}{*}{\textbf{LLaMa2-Chat-INT4}} & S: CNN/Daily     & 100          &              & 100           \\
%                                            & QA: SQuAD        & 100          & 3.4          & 100           \\
%                                            & QA: Truthful\_QA & 100          & 4.7          & 100           \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:my-table}
% \end{table}

==> table-inference-breakdown.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{l|rrr|rrr|rrr}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{r|}{Ideal}                               & \multicolumn{3}{r|}{Layer-holding}                                     & \multicolumn{3}{r}{Layer-swapping}                                     \\ \cline{2-10} 
                       & \multicolumn{1}{r|}{C}   & \multicolumn{1}{r|}{WL} & R   & \multicolumn{1}{r|}{C}   & \multicolumn{1}{r|}{WL}    & R              & \multicolumn{1}{r|}{C}   & \multicolumn{1}{r|}{WL}    & R              \\ \hline
GPT2                   & \multicolumn{1}{r|}{191} & \multicolumn{1}{r|}{0}  & 0\% & \multicolumn{1}{r|}{234} & \multicolumn{1}{r|}{11778} & \textbf{1.9\%} & \multicolumn{1}{r|}{240} & \multicolumn{1}{r|}{14214} & \textbf{1.6\%} \\ \hline
T5                     & \multicolumn{1}{r|}{72}  & \multicolumn{1}{r|}{0}  & 0\% & \multicolumn{1}{r|}{81}  & \multicolumn{1}{r|}{7017}  & \textbf{1.1\%} & \multicolumn{1}{r|}{91}  & \multicolumn{1}{r|}{7208}  & \textbf{1.2\%} \\ \hline
mT5                    & \multicolumn{1}{r|}{92}  & \multicolumn{1}{r|}{0}  & 0\% & \multicolumn{1}{r|}{128} & \multicolumn{1}{r|}{7086}  & \textbf{1.8\%} & \multicolumn{1}{r|}{164} & \multicolumn{1}{r|}{7521}  & \textbf{2.1\%} \\ \hline
\end{tabular}%
}
\caption{Different models inference latency (ms) breakdown. C, WL, and R represent computing, weights loading, and computing-inference ratio, respectively. }
\label{table-breakdown}
\end{table}

==> table-processor-utilization.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{l|l|r|r}
\hline
Device                           & Models     & Ideal & Layer-swapping \\ \hline
\multirow{3}{*}{GPU on TX2}      & GPT2-Large &                      &                \\ \cline{2-5} 
                                 & mT5-Large  &                      &   16.5\%       \\ \cline{2-5} 
                                 & T5-Large   &                      &                \\ \hline
\multirow{2}{*}{CPU on xiaomi10} & LLaMa-13B  &                      &                \\ \cline{2-5} 
                                 & GLM-33B    &                      &                \\ \hline
\end{tabular}%
}
\caption{Average processor utilization when inferring target model.}
\label{table-processor-utilization}
\end{table}
